Dynamic Tensor Rematerialization

Checkpointing enables the training of deep learning models under restricted memory budgets by freeing intermediate activations from memory and recomputing them on demand. Current checkpointing techniques statically plan these recomputations offline and assume static computation graphs. We demonstrate that a simple online algorithm can achieve comparable performance by introducing Dynamic Tensor Rematerialization (DTR), a greedy online algorithm for checkpointing that is extensible and general, is parameterized by eviction policy, and supports dynamic models. We prove that DTR can train an $N$-layer linear feedforward network on an $\Omega(\sqrt{N})$ memory budget with only $\mathcal{O}(N)$ tensor operations. DTR closely matches the performance of optimal static checkpointing in simulated experiments. We incorporate a DTR prototype into PyTorch merely by interposing on tensor allocations and operator calls and collecting lightweight metadata on tensors.

==> background.tex <==
\section{Background}

In this section,
we will review in more detail
the typical architecture for a DL model
as well as the process for training models.
We will then discuss
the types of more dynamic models
that have arisen for natural language processing applications
and how they deviate from the conventions of static models.

\subsection{Neural Network Definitions}

The typical form for a DL model is a neural network,
formed as a directed acyclic graph with
a number of input nodes and one output node,
with nodes called ``neurons'' between them.
The inputs to a neural network and its outputs
are typically tensors.
Neurons correspond to arithmetic operations,
while edges correspond to dataflow relations:
an edge from node $n_1$ to node $n_2$
signifies that the output
of the operation performed at $n_1$
is passed as input
to the operation performed at $n_2$.
Typically, each neuron (and the output node)
performs a nonlinear operation $\phi$
on a weighted sum of its inputs, $\phi(\Sigma w_i v_i)$,
so each edge in the network has an associated weight
(neurons do not all need to perform the same operation).
The edge weights thus comprise the parameters of the network;
since the inputs and output of the network are tensors
and there can be many edges,
most neural networks have many parameters.
Neural networks are usually organized in ``layers''
such that
the input nodes form the first layer,
the output node forms the last,
and the neurons form a number of layers
(called ``hidden layers'')
where each neuron in each layer
has an incoming edge from each node in the preceding layer
and has an outgoing edge to each node in the next layer.
If all the weights of the network are set,
the network can be evaluated layer by layer
starting from the input nodes
and proceeding until the output node is evaluated:
each node in a layer receives its inputs,
computes its result,
and sends the result to the nodes of the following layer.


Many models that have achieved high accuracy in vision tasks
are static neural networks with many layers,
such as variants of the Deep Residual Network (ResNet)~\cite{resnet}.

\subsection{Training}

As neural networks operate over numbers and produce numbers,
applying a neural network
to a particular problem in some domain
requires expressing
the problem in terms of numerical inputs to the network,
interpreting the network's numerical output,
and choosing appropriate parameters for the network
so that it computes the intended outputs.
Neural networks generally have too many parameters
for them to be chosen manually,
especially if the networks operate over large tensors.
Parameters can instead be chosen automatically
given labeled examples (pairs of input with expected output)
by treating the choice of parameters
as an optimization problem:
Given some cost function
comparing the network's output with the expected output,
find parameters that minimize the cost (often called the ``loss'')
for the given inputs.
The process of choosing parameters based on labeled examples
is called ``training.''

Training is usually done by variants of gradient descent,
a process in which the network under candidate parameters
is evaluated against the inputs in several epochs until fixpoint;
in each epoch,
the total loss and the gradient of the loss function
(with respect to the parameters)
are used to update the parameters for the next epoch,
adjusting the parameters in the opposite direction of the gradient.
Gradient descent
and variants like stochastic gradient descent (the most commonly used)
require that the loss function be differentiable
and that there be a way to update the parameters
given the loss and gradient.
In the case of neural networks,
if each neuron's operation is differentiable,
then the entire network is differentiable (as is the loss function);
moreover, the individual neurons' partial derivatives
can be used to systematically adjust the parameters
in a process called ``backpropagation.''
In backpropagation, the parameters for a given neuron
are adjusted based on that neuron's contribution to the error,
which depends on the error from the following layer,
the total gradient,
the neuron's partial derivative with respect to a parameter,
and the results of the neuron when evaluating the inputs
(called the ``activation''),
moving ``backwards'' starting from the network's output.
Of most relevance to the topic of checkpointing,
backpropagation requires storing intermediate activations
for the entire network,
which contributes greatly to the memory load
of training a neural network.

Models must often be trained on very large datasets
to obtain high accuracy in real-world tasks;
for example, ImageNet~\cite{imagenet_cvpr09},
a common benchmark for training image recognition models,
contains millions of images divided into thousands of categories.

\subsection{Dynamic Models}

In many applications,
especially in the domain of natural language processing,
the order of sequential inputs can encode important information
(e.g., ``The cat chased the dog" versus ``The dog chased the cat").
Handling sequential input in a deep learning model
requires a different design from the static computation graphs
used in vision applications,
as those usually handle fixed-size inputs
without such ordering constraints.
A recurrent neural network (RNN)
is a type of model
designed to handle variable-length sequential input
and take ordering into account.
Unlike most vision models,
RNNs feature data-dependent control flow,
looping over the input sequence
and producing an output sequence
while passing some amount of internal state
(called the ``hidden state") between loop iterations.
The loop body is known as an RNN ``cell''
and generally consists of tensor operators
like those that would be found in a static neural network.
In each iteration,
the RNN cell takes a member of the sequence
and the previous hidden state
and produces an output and a new hidden state.
The hidden state serves as context
that allows earlier entries in the sequence
to provide information for processing later entries.

An RNN of particular interest is the TreeLSTM~\cite{tree_lstm},
which is a generalization of an RNN with an LSTM (Long Short-Term Memory) cell
to handle tree-structured input with arbitrary branching.
A tree-structured RNN like TreeLSTM
recurses down the input tree,
applying the cell and updating the hidden state
according to a traversal order,
rather than simply looping in sequence.
When the input is, for example, a grammatical parse tree,
the branching of the tree can encode information
about the significance of different parts of the input,
which the TreeLSTM can take into account.
Accordingly, TreeLSTMs and related models
have achieved strong results on many NLP tasks,
such as sentiment analysis.

Certain models recently introduced for linguistic reasoning tasks
feature an even greater degree of dynamic control flow.
For example, the Neuro-Symbolic Concept Learner~\cite{neuro_symbolic} (NS-CL)
can learn a structured representation of an image
based on question-answer pairs about it.
The NS-CL was used to obtain state-of-the-art results
on a visual question-answering task
with an architecture in many stages
where the output of one stage
can affect the control flow in another.
In the NS-CL, a vision model takes an image as input
and produces a structured representation of it,
while an RNN encodes questions
that are then decoded
into queries about the image representation
that are handled by a differentiable executor.
Since the learner's answers to questions about an image
can be affected not only by the content of the images and the questions
but also by the data structures produced by the vision model and question decoder,
which depend on model parameters.

Training dynamic models by stochastic gradient descent
is often more involved than for static neural networks,
as the amount of computation performed can differ
based on the inputs or the parameters.
This means that
knowing the derivatives for individual tensor operations
in the model's description
(e.g., the operators in an RNN cell)
is not alone sufficient to find the gradient for the model;
the number of iterations and the dependencies between them
are also relevant.
Hence, backpropagation
as described for neural networks
does not directly generalize to dynamic models.
In some cases, it may be possible to ``unroll'' RNNs
and turn them into static networks
if there is a known bound on the input size,
but this must often be done manually
and requires padding out shorter inputs;
models like NS-CL,
where parameters can affect control flow,
cannot be unrolled.
Reverse-mode automatic differentiation (AD),
which can account for arbitrary control flow,
can be used to more generally find gradients for dynamic models.
Like backpropagation, reverse-mode AD
requires storing intermediate values produced by the model;
most implementations keep a record
of the complete computation as it unfolds
called a ``Wengert list'' or ``tape,''
storing the intermediate values
for handling different differentiation rules.

Note, however,
that recently a class of models
has been able to obtain high accuracy
on natural language processing tasks
dealing with sequential inputs
\textit{without} data-dependent control flow.
These models are variants of Transformer,
introduced in~\cite{attention_is_all_you_need},
which assume a maximum sequence length
and utilize an ``attention mechanism''
to take the values of particular elements in the sequence
(indexing into the sequence like a pointer,
but in a manner that is still differentiable)
and pass weighted sums to encoder and decoder mechanisms.
As Vaswani \textit{et al.} note,
the attention mechanism removes
the sequential dependency present in RNNs
and allows for more of the model to be computed in parallel.
The original model introduced in~\cite{attention_is_all_you_need}
was able to achieve state-of-the-art results
on a sequence-to-sequence translation task
and further models using attention mechanisms
have since made progress on other problems.
While these attention-based models
do not have data-dependent control flow,
some existing checkpointing algorithms cannot handle
Transformer and related models
because the encoder and decoder mechanisms
feature tensor \textit{shapes} that depend on the input.
